Revisiting Differentially Private Hypothesis Tests for Categorical Data

In this paper, we consider methods for performing hypothesis tests on data protected by a statistical disclosure control technology known as differential privacy. Previous approaches to differentially private hypothesis testing either perturbed the test statistic with random noise having large variance (and resulted in a significant loss of power) or added smaller amounts of noise directly to the data but failed to adjust the test in response to the added noise (resulting in biased, unreliable $p$-values). In this paper, we develop a variety of practical hypothesis tests that address these problems. Using a different asymptotic regime that is more suited to hypothesis testing with privacy, we show a modified equivalence between chi-squared tests and likelihood ratio tests. We then develop differentially private likelihood ratio and chi-squared tests for a variety of applications on tabular data (i.e., independence, sample proportions, and goodness-of-fit tests). Experimental evaluations on small and large datasets using a wide variety of privacy settings demonstrate the practicality and reliability of our methods.

==> appsens.tex <==
We now provide $s_h$ calculations for the output perturbation versions of the test statistics. In some cases, $s_h$ depends on the dimensions of $T$. 
\ConfOrTech{Due to space constraints, we present the most important $s_h$ results. The full results and proofs can be found in the long version \cite{wang2015differentially}.}{Proofs can be found in Appendix \ref{sec:sensitivityproofs}.} One important fact to note is that the Diff statistic has lowest $s_h$ and so, intuitively, is expected to perform well in the privacy setting.

%\subsubsection{Output Perturbation Methods} \label{subsec:outputperturb}
%Using the permutation testing framework with output perturbation means that we need to derive the sensitivity (Definition \ref{def:sensitivity}) for each test statistic and add Laplace noise with variance that depends on the sensitivity. The results are presented in this section. In general, results for $2\times 2$ tables have additional mathematical cancellations in their computation and so they differ from tables with dimensions $3\times 3$ or larger, which do not have these cancellations. Generally, sensitivity depends on the actual (known) marginals and is greatly affected by rows and columns with low counts. The exception is the \varchi{statistic}, which has constant sensitivity regardless of the values of the marginals. Furthermore, under the null hypothesis, the \varchi{statistic} grows with $n$ and will eventually overwhelm the Laplace noise (as is the case for statistics using input perturbation). The log-likelihood statistic will also overwhelm the noise. However, classical statistics (chi-squared and likelihood ratio)  do not have this property. This again suggests that privacy considerations fundamentally change how we should perform data analysis. 

%The proofs of the following theorems are omitted due to space constraints but are available upon request.

%In order to perturb the test statistics, we need to compute their sensitivities. More specially, sensitivities based on neighboring contingency tables with fixed marginals, which are stated through the following theorems. 
%Note we have separate sensitivity results for $\chi^2$-statistic on $2 \times 2$ contingency tables and general contingency tables (larger than $2 \times 2$) since the sensitivity for $2 \times 2$ contingency tables are asymptotically constant, which is not true for larger tables.

\techreport{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}{theorem}{cssensitivitytwo}
\label{thm:chi2sensitivity2by2}
 The $s_h$ value of the $\chi^2$-statistic for a $2 \times 2$ contingency tables is: 
 {\small
 \begin{align*}
  \max
  \begin{cases}
   C\left|n-2T[\cdot,2]T[1,\cdot]\right| & \text{if $T[1,\cdot] \leq T[\cdot,1]$, $T[2,\cdot] \geq T[\cdot,2]$} \\
   C\left|n-2T[\cdot,1]T[2,\cdot]\right| & \text{if $T[1,\cdot] > T[\cdot,1]$, $T[2,\cdot] < T[\cdot,2]$} \\
   C\left|n-2T[\cdot,1]T[1,\cdot]\right| & \text{if $T[1,\cdot] \leq T[\cdot,2]$, $T[2,\cdot] \geq T[\cdot,1]$} \\
   C\left|n-2T[\cdot,2]T[2,\cdot]\right| & \text{if $T[1,\cdot] > T[\cdot,2]$, $T[2,\cdot] < T[\cdot,1]$}
  \end{cases}
 \end{align*}
 }
 where $C=\frac{n^2}{T[\cdot,1]T[\cdot,2]T[1,\cdot]T[2,\cdot]}$.
\end{restatable}
The Proof of Theorem~\ref{thm:chi2sensitivity2by2} is provided in Appendix~\ref{subsec:chi2sensitivity2by2}.
Note that table margins are $O(n)$, so the constant $C$ in Theorem~\ref{thm:chi2sensitivity2by2} is $O(1/n^2)$ and so the $s_h$ value is $O(1)$ for $2\times 2$ tables. However, the chi-squared statistic does not grow with $n$ under the null hypothesis, so the noise can be a significant part of the output.

}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{restatable}{theorem}{cssensitivity}
\label{thm:chi2sensitivity}
 The $s_h$ value of the $\chi^2$-statistic for an $r \times c$ table $T$ with $r \geq 3$, $c \geq 3$ is:
$$
  \max
  \begin{cases}
   \max\limits_{i_1,i_2,j_1,j_2}C'\Big|2(T[i_2,\cdot]T[\cdot,j_2]a+T[i_1,\cdot]T[\cdot,j_1]d)-
   (T[i_1,\cdot]+T[i_2,\cdot])(T[\cdot,j_1]+T[\cdot,j_2])\Big|/n
   \\
   \max\limits_{i_1,i_2,j_1,j_2}C'\Big|(T[i_1,\cdot]-T[i_2,\cdot])(T[\cdot,j_1]-T[\cdot,j_2])-
    2(T[i_2,\cdot]T[\cdot,j_1]b+T[i_1,\cdot]T[\cdot,j_2]c)\Big|/n
  \end{cases}
$$
 where $a=\min(T[i_1,\cdot],T[\cdot,j_1])$, $d=\min(T[i_2,\cdot],T[\cdot,j_2])$, $b=\min(T[i_1,\cdot],T[\cdot,j_2])-1$, $c=\min(T[i_2,\cdot],T[\cdot,j_1])-1$ and $C'=\frac{n^2}{T[\cdot,j_1]T[\cdot,j_2]T[i_1,\cdot]T[i_2,\cdot]}$.
\end{restatable}
\techreport{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
The proof of Theorem~\ref{thm:chi2sensitivity} is provided in Appendix~\ref{subsec:chi2sensitivity}.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\techreport{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A simple analysis shows that the $s_h$ in Theorem \ref{thm:chi2sensitivity} is $O(1)$.

\begin{restatable}{theorem}{lrsensitivitytwo} 
\label{thm:lrsensitivity2by2}
 The $s_h$ value of the likelihood ratio statistic for $2 \times 2$ contingency tables is
\begin{align*}
  2 \times \max
  \begin{cases}
   \left|\log\frac{T[1,\cdot]^{T[1,\cdot]}}{(T[1,\cdot]-1)^{T[1,\cdot]-1}} + \log\frac{T[\cdot,2]^{T[\cdot,2]}}{(T[\cdot,2]-1)^{T[\cdot,2]-1}} +
   \log\frac{(T[2,\cdot]-T[\cdot,2])^{T[2,\cdot]-T[\cdot,2]}}{(T[2,\cdot]-T[\cdot,2]+1)^{T[2,\cdot]-T[\cdot,2]+1}}\right|
   \\
   \text{if $T[1,\cdot] \leq T[\cdot,1]$, $T[2,\cdot] \geq T[\cdot,2]$}
   \\
   \left|\log\frac{T[2,\cdot]^{T[2,\cdot]}}{(T[2,\cdot]-1)^{T[2,\cdot]-1}} + \log\frac{T[\cdot,1]^{T[\cdot,1]}}{(T[\cdot,1]-1)^{T[\cdot,1]-1}} +
   \log\frac{(T[\cdot,2]-T[2,\cdot])^{T[\cdot,2]-T[2,\cdot]}}{(T[\cdot,2]-T[2,\cdot]+1)^{T[\cdot,2]-T[2,\cdot]+1}}\right|
   \\
   \text{if $T[1,\cdot] > T[\cdot,1]$, $T[2,\cdot] < T[\cdot,2]$}
   \\
   \left|\log\frac{(T[1,\cdot]-1)^{T[1,\cdot]-1}}{T[1,\cdot]^{T[1,\cdot]}} + \log\frac{(T[\cdot,1]-1)^{T[\cdot,1]-1}}{T[\cdot,1]^{T[\cdot,1]}} +
   \log\frac{(T[2,\cdot]-T[\cdot,1]+1)^{T[2,\cdot]-T[\cdot,1]+1}}{(T[2,\cdot]-T[\cdot,1])^{T[2,\cdot]-T[\cdot,1]}}\right|
   \\
   \text{if $T[1,\cdot] \leq T[\cdot,2]$, $T[2,\cdot] \geq T[\cdot,1]$}
   \\
   \left|\log\frac{(T[2,\cdot]-1)^{T[2,\cdot]-1}}{T[2,\cdot]^{T[2,\cdot]}} + \log\frac{(T[\cdot,2]-1)^{T[\cdot,2]-1}}{T[\cdot,2]^{T[\cdot,2]}} +
   \log\frac{(T[1,\cdot]-T[\cdot,2]+1)^{T[1,\cdot]-T[\cdot,2]+1}}{(T[1,\cdot]-T[\cdot,2])^{T[1,\cdot]-T[\cdot,2]}}\right|
   \\
   \text{if $T[1,\cdot] > T[\cdot,2]$, $T[2,\cdot] < T[\cdot,1]$}
  \end{cases}
\end{align*}
\end{restatable}
The proof of Theorem~\ref{thm:lrsensitivity2by2} is provided in Appendix~\ref{subsec:lrsensitivity2by2}.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{restatable}{theorem}{lrsensitivity} 
\label{thm:lrsensitivity}
 The $s_h$ of the likelihood ratio statistic LR on $r \times c$ ($r \geq 3$, $c \geq 3$) contingency tables is
 \begin{displaymath}
  2 \times \max
   \left\{\max\limits_{i_1,i_2,j_1,j_2}\left[\log\frac{a^a}{(a-1)^{a-1}} + \log\frac{d^d}{(d-1)^{d-1}}\right],
   \max\limits_{i_1,i_2,j_1,j_2}\left[\log\frac{(b+1)^{b+1}}{b^b} + \log\frac{(c+1)^{c+1}}{c^c}\right]\right\}
 \end{displaymath}
 where $a=\min(T[i_1,\cdot],T[\cdot,j_1])$, $d=\min(T[i_2,\cdot],T[\cdot,j_2])$, $b=\min(T[i_1,\cdot],T[\cdot,j_2])-1$, $c=\min(T[i_2,\cdot],T[\cdot,j_1])-1$.
\end{restatable}
\techreport{The proof of Theorem~\ref{thm:lrsensitivity} is provided in Appendix~\ref{subsec:lrsensitivity}.}
Thus $s_h = O(\log n)$ while the statistic itself does not grow with $n$ under the null hypothesis.

%From Theorems \ref{thm:lrsensitivity2by2} and \ref{thm:lrsensitivity}, it is clear that the sensitivity is $O(\log(n))$. Meanwhile, under the null hypothesis, the value of the test statistic does not grow with $n$.
%\begin{restatable}{theorem}{lrsensitivityub} 
%\label{thm:lrsensitivityub}
% The sensitivity of the likelihood ratio statistic based on contingency tables no smaller than $2 \times 2$ with fixed marginals %is upper bounded by $2n\log
% \frac{n}{n-2}+4\log\frac{n-2}{2}$.
%\end{restatable}
%\techreport{The proof of Theorem~\ref{thm:lrsensitivityub} is provided in Appendix~\ref{pf:lrsensitivityub}}.

\techreport{%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}{theorem}{llsensitivitytwo}
\label{thm:llsensitivity2by2}
 The $s_h$ value of the log-likelihood statistic based on $2 \times 2$ contingency tables is
 \begin{equation*}
  \max
  \begin{cases}
   \left|\log(T[2,\cdot]-T[\cdot,2]+1)-\log T[1,\cdot]-\log T[\cdot,2]\right|
   \quad\text{if $T[1,\cdot] \leq T[\cdot,1]$, $T[2,\cdot] \geq T[\cdot,2]$}
   \\
   \left|\log(T[\cdot,2]-T[2,\cdot]+1)-\log T[2,\cdot]-\log T[\cdot,1]\right|
    \quad\text{if $T[1,\cdot] > T[\cdot,1]$, $T[2,\cdot] < T[\cdot,2]$}
   \\
   \left|\log T[1,\cdot]+\log T[\cdot,1]-\log(T[2,\cdot]-T[\cdot,1]+1)\right|
    \quad\text{if $T[1,\cdot] \leq T[\cdot,2]$, $T[2,\cdot] \geq T[\cdot,1]$}
   \\
   \left|\log T[2,\cdot]+\log T[\cdot,2]-\log(T[1,\cdot]-T[\cdot,2]+1)\right|
    \quad\text{if $T[1,\cdot] > T[\cdot,2]$, $T[2,\cdot] < T[\cdot,1]$}
  \end{cases}
 \end{equation*}
\end{restatable}
The proof of Theorem~\ref{thm:llsensitivity2by2} is provided in Appendix~\ref{subsec:llsensitivity2by2}.
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{restatable}{theorem}{llsensitivity}
\label{thm:llsensitivity}
 The $s_h$ value of the LL statistic (from Equation~\ref{eqn:lldef}) for $r \times c$ tables ($r \geq 3$, $c \geq 3$) is
 \begin{equation*}
  \max\left\{\max\limits_{i_1,i_2,j_1,j_2}\log\left[(b+1)(c+1)\right], \max\limits_{i_1,i_2,j_1,j_2}\log\left(ad\right)\right\}
 \end{equation*}
 where $a=\min(T[i_1,\cdot],T[\cdot,j_1])$, $d=\min(T[i_2,\cdot],T[\cdot,j_2])$, $b=\min(T[i_1,\cdot],T[\cdot,j_2])-1$, $c=\min(T[i_2,\cdot],T[\cdot,j_1])-1$.
\end{restatable}
\techreport{The proof of Theorem~\ref{thm:llsensitivity} is provided in Appendix~\ref{subsec:llsensitivity}.}
Here $s_h$ also grows logarithmically. %However since the test statistic is the log probability of a table under the hypergeometric distribution, this test statistic grows with $n$ and so the data should eventually overwhelm the added Laplace noise.
%\begin{restatable}{theorem}{llsensitivityub}
%\label{thm:llsensitivityub}
% The sensitivity of the log-likelihood statistic based on contingency tables no smaller than $2 \times 2$ with fixed marginals is upper bounded by $2\log\frac{n}{2}$.
%\end{restatable}
%\techreport{The proof of Theorem~\ref{thm:llsensitivityub} is provided in Appendix~\ref{pf:llsensitivityub}}.

\begin{restatable}{theorem}{absolutediffsensitivity}
\label{thm:absolutediffsensitivity}
 The $s_h$ value of the Diff statistic (from Equation~\ref{eqn:diffdef}) is equal to $4$.
\end{restatable}
\techreport{Proof of Theorem~\ref{thm:absolutediffsensitivity} is provided in \ConfOrTech{additional materials.}{Appendix~\ref{subsec:absolutediffsensitivity}.}}
All proofs can be found in \cite{wang2015differentially}. The Diff statistic is the only one out of them that has a constant sensitivity. Clearly the value of the statistic should grow with $n$, even under the null distribution, so it should quickly  overwhelm the Laplace noise.


%The sensitivity of $\chi^2$-statistic on general contingency tables with fixed marginals grows linearly with sample size, which means getting more data does not help to improve the utility of differentially private hypothesis testing. Also, adding noise according to this sensitivity can dominate the actual test statistic. For likelihood ratio statistic and log-likelihood statistic, their sensitivities grow logarithmically with sample size. Although the sensitivities are much smaller, we can still show this can lead to terrible results for the tests. Example~\ref{eg:fn} and \ref{eg:fp} show that with log-linear sensitivity, the result of the hypothesis test can be completely incorrect with high probability.

%\begin{example} \label{eg:fn}
% The likelihood ratio statistic based on the left table in Table~\ref{tab:1} is $10.4818$, the $p$-value is $0.0012$. With significance level $\alpha=0.05$, we reject the null hypothesis. Now we show there is high probability of false negative when noise is added. The global sensitivity of likelihood ratio statistic based on neighboring contingency tables with fixed marginals is $28.85$ when $n=1000$. Let $\epsilon=1.0$ which is a pretty relaxed privacy guarantee, then the noise parameter is $28.85$. The probability of getting a false negative when Laplace noise is added to the test statistic is approximately $0.397$. 
%\end{example}

%\begin{example} \label{eg:fp}
% The likelihood ratio statistic based on the right table in Table~\ref{tab:1} is $2.7070$, the $p$-value is $0.0999$. With significance level $\alpha=0.05$, we can not reject the null hypothesis. Now we show there is high probability of false positive when noise is added. Let $\epsilon=1.0$, with the same global sensitivity analysis, we get the same noise parameter $28.85$. The probability of getting a false positive when Laplace noise is added to the test statistic is approximately $0.481$.
%\end{example}

%\begin{table}
% \centering
% \caption{Two Sample Contingency Tables Used to Demonstrate Sensitivity Analysis} 
% \label{tab:1}
% \subfloat{
%  %\caption{}
%  %\label{tab:1a}
%  \begin{tabular}{|c|c|}
%   \hline
%   281 & 234 \\
%   \hline
%   215 & 270 \\
%   \hline
%  \end{tabular}
% }
% \hfil
% \subfloat{
%  %\centering
%  %\caption{}
%  %\label{tab:1b}
%  \begin{tabular}{|c|c|}
%   \hline
%   263 & 239 \\
%   \hline
%   235 & 263 \\
%   \hline
%  \end{tabular}
% }
%\end{table}

%It is easy to see the sensitivity of the \varchi{statistic} based on contingency tables with fixed marginals is $4$, which is constant. Therefore we expect the \varchi{test} to outperform others in the noisy case.
%
%Given a general contingency table, when we double each cell count, all the four test statistics on the new table are doubled. Based on contingency tables with fixed marginals, the sensitivity of $\chi^2$-statistic is doubled, the sensitivities of likelihood ratio statistic and log-likelihood statistic increase by some constant. The sensitivity of the \varchi{statistic} does not change.

%\subsection{Input Perturbation Methods} \label{subsec:inputperturb}
%With input perturbation, we add noise to the entries of the contingency table based on Laplace mechanism. Since we are considering neighboring contingency tables with fixed marginals, the sensitivity of releasing the contingency table is $4$. To maintain the marginal sums, we perturb all the cell counts except those from the last row and last column, and use the marginal sums to figure out the rest cell counts. However, this may lead to negative cell counts in the noisy table. We then apply least squares consistency mechanism on the noisy table to get a consistent one with the same marginals and no negative cell counts such that the square distance between the perturbed cell counts from the two tables is minimized.
%
%Let $T$ be the $r \times c$ original contingency table, $\widehat{T}$ be the noisy contingency table after adding noise (to the cells except those from the last row and last column), $T_b$ be the consistent noisy table with no negative cell counts (the subscript $b$ indicates we bound the table to exclude negative numbers). Let $x, \widehat{x}, x_b$ be the vector representation of $T, \widehat{T}, T_b$ respectively. Let $Ax=d$ be the fixed marginals constraint. Let $x_b \geq 0$ be the non-negativity constraint. 
%
%Define $H$ to be a $(r-1)(c-1) \times rc$ matrix such that $Hx$ gives the vector representation of $T$ without entries from its last row and last column. 
%$$H[i,j]=
%\begin{cases}
% 1 & \quad \text{$i \in [(k-1)(c-1)+1,k(c-1)]$ and}\\
%   & \quad \text{$j=i+k-1$ where $k \in [1,r-1]$} \\
% 0 & \quad \text{otherwise}
%\end{cases}
%$$
%
%We solve the following problem for $x_b$:
%\begin{displaymath} 
% \min_{x_b}\frac{1}{2}\left|\left|H\widehat{x}-Hx_b\right|\right|_2^2 \quad\text{s.t. $Ax_b=d$, $x_b\geq0$}
%\end{displaymath}
%
%We use KKT conditions to solve the constrained least squares problem with both equality and inequality constraints. Then we can get $T_b$ from $x_b$. 
%
%These consistent noisy contingency tables can be released without privacy breach. Computing test statistics from these contingency tables also preserves differential privacy. 
%
%\subsection{Permutation Test} \label{subsec:permutationtest}
%We have shown how to get differentially private test statistics for independence testing. Next, we estimate $p$-values from these noisy test statistics through permutation test.
%
%A permutation is a random rearrangement of the elements in the data. A permutation of a contingency table with fixed marginals is a rearrangement of the cell counts with unchanged marginals. For example, $[[8,32],[42,18]]$ is a permutation of $[[25,15],[25,35]]$.
%
%Given a contingency table, we can run the algorithm Permutation Test in Figure~\ref{alg:permutationtest} to estimate its $p$-value for a certain test, which is computed by the fraction of test statistics from the permutations which are no less than the test statistic computed from the original table.

%\begin{algorithm}[!t]
% \LinesNumbered
% \DontPrintSemicolon
% \SetAlgoLined
% \SetKwInOut{Input}{input}
% \SetKwInOut{Output}{output}
% \begin{lrbox}{\mybox}
% \begin{minipage}{\hsize}
% \textbf{Algorithm} Permutation Test\;
%
% \Input{A contingency table $T$, number of permutations $m$, test statistic $ts$}
% \Output{Estimated $p$-value of $T$}
% \For{$i \leftarrow 1$ \KwTo $m$}{
%     $/*$ \textit{get a permutation of $T$} $*/$\;
% 
%     $D \leftarrow Array(1, 2, \dots, n)$\;
% 
%     $counter \leftarrow 0$\;
% 
%     \For{$j \leftarrow 1$ \KwTo $r$}{
%         $/*$ \textit{assign attribute value of the the first attribute for each element} $*/$\;
%     
%         \For{$k \leftarrow counter$ \KwTo $counter+T[j,\cdot]$}{
%             $A_{1}[D[k]] \leftarrow j$\;
%         }
%     
%         $counter \leftarrow counter+T[j,\cdot]$\;
%     }
% 
%     shuffle $D$, get $D'$\;
% 
%     $counter \leftarrow 0$\;
% 
%     \For{$j \leftarrow 1$ \KwTo $c$}{
%
%         $/*$ \textit{assign attribute value of the the second attribute for each element} $*/$\;
%     
%         \For{$k \leftarrow counter$ \KwTo $counter+T[\cdot,j]$}{
%             $A_{2}[D'[k]] \leftarrow j$\;
%         }
%
%         $counter \leftarrow counter+T[\cdot,j]$\;
%     }
% 
%     $R_i \leftarrow$ contingency table of the elements based on $A_1, A_2$\;
% }
% 
% output $\left|ts(R_i): ts(R_i) \geq ts(T)\right| / m$
% \end{minipage}%
% \end{lrbox}
% \hspace*{-10pt}\framebox[\columnwidth]{\hspace*{15pt}\usebox\mybox\par}
% \caption{Permutation test}
% \label{alg:permutationtest}
%\end{algorithm}
